Do I have the Knowledge to Answer? Investigating Answerability of Knowledge Base Questions

When answering natural language questions over knowledge bases, missing facts, incomplete schema and limited scope naturally lead to many questions being unanswerable. While answerability has been explored in other QA settings, it has not been studied for QA over knowledge bases (KBQA). We create GrailQAbility, a new benchmark KBQA dataset with unanswerability, by first identifying various forms of KB incompleteness that make questions unanswerable, and then systematically adapting GrailQA (a popular KBQA dataset with only answerable questions). Experimenting with three state-of-the-art KBQA models, we find that all three models suffer a drop in performance even after suitable adaptation for unanswerable questions. In addition, these often detect unanswerability for wrong reasons and find specific forms of unanswerability particularly difficult to handle. This underscores the need for further research in making KBQA systems robust to unanswerability

==> checklist.tex <==

A. For every submission:\\
A1. Did you describe the limitations of your work? {\bf Yes.}\\
%Point out any strong assumptions and how robust your results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only held locally). Reflect on how these assumptions might be violated in practice and what the implications would be.
%Reflect on the scope of your claims, e.g., if you only tested your approach on a few datasets, languages, or did a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated. Reflect on the factors that influence the performance of your approach. For example, a speech-to-text system might not be able to be reliably used to provide closed captions for online lectures because it fails to handle technical jargon.
%If you analyze model biases: which definition of bias are you using? Did you state the motivation and definition explicitly? See the discussion in Blodgett et al. (2020).
%We understand that authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection. It is worth keeping in mind that a worse outcome might be if reviewers discover limitations that aren’t acknowledged in the paper. In general, we advise authors to use their best judgement and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
A2. Did you discuss any potential risks of your work? {\bf Yes}\\
%Examples of risks include potential malicious or unintended harmful effects and uses (e.g., disinformation, generating fake profiles, surveillance), environmental impact (e.g., training huge models), fairness considerations (e.g., deployment of technologies that could further disadvantage or exclude historically disadvantaged groups), privacy considerations (e.g., a paper on model/data stealing), and security considerations (e.g., adversarial attacks). See discussion in Leins et. al. (2020) as examples.
%Does the research contribute to overgeneralization, bias confirmation, under or overexposure of specific languages, topics, or applications at the expense of others? See Hovy and Spruit (2016) for examples.
%We expect many papers to be foundational research and not tied to particular applications, let alone deployments. However, we encourage authors to discuss potential risks if they see a path to any positive or negative applications. For example, the authors can emphasize how their systems are intended to be used, how they can safeguard their systems against misuse, or propose future research directions.
%Consider different stakeholders that could be impacted by your work. Is it possible that research benefits some stakeholders while harming others? Does it pay special attention to vulnerable or marginalized communities? Does the research lead to exclusion of certain groups? See Dev et. al (2021) for examples.
%Consider dual use, i.e, possible benefits or harms that could arise when the technology is being used as intended and functioning correctly, benefits or harms that could arise when the technology is being used as intended but gives incorrect results, and benefits or harms following from (intentional or unintentional) misuse of the technology.
%Consider citing previous work on relevant mitigation strategies for the potential risks of the work (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of NLP).
A3. Do the abstract and introduction summarize the paper’s main claims? {\bf Yes}\\
%The main claims in the paper should be clearly stated in the abstract and in the introduction.
%These claims should be supported by evidence presented in the paper, potentially in the form of experimental results, reasoning, or theory. The connection between which evidence supports which claims should be clear.
%The context of the contributions of the paper should be clearly described, and it should be stated how much the results would be expected to generalize to other contexts.
%It should be easy for a casual reader to distinguish between the contributions of the paper and open questions, future work, aspirational goals, motivations, etc.
B. Did you use or create scientific artifacts? {\bf Yes}\\
%Scientific artifacts may include code, data, models or other artifacts.
%Most NLP research uses scientific artifacts.
%Many NLP papers are accompanied by new scientific artifacts.
B1. Did you cite the creators of artifacts you used? {\bf Yes}\\
%For composite artifacts like the GLUE benchmark, this means all creators.
%Cite the original paper that produced the code package or dataset.
%Remember to state which version of the asset you’re using.
%If possible, include a URL.
B2. Did you discuss the license or terms for use and / or distribution of any artifacts?\\
%State the name of the license (e.g., CC-BY 4.0) for each asset.
%If you scraped or collected data from a particular source (e.g., website or social media API), you should state the copyright and terms of service of that source. Please note that some sources do not allow inference of protected categories like gender, sexual orientation, health status, etc.
%The data might be in public domain and licensed for research purposes.
%The data might be used with consent of its creators or copyright holders.
%If the data is used without consent, the paper makes the case to justify its legal basis (e.g., research performed in the public interest under GDPR).
%If you are releasing assets, you should include a license, copyright information, and terms of use in the package.
%If you are repackaging an existing dataset, you should state the original license as well as the one for the derived asset (if it has changed).
%If you cannot find this information online, you are encouraged to reach out to the asset’s creators.
B3. Did you discuss if your use of existing artifact(s) was consistent with their intended use, provided that it was specified? For the artifacts you create, do you specify intended use and whether that is compatible with the original access conditions (in particular, derivatives of data accessed for research purposes should not be used outside of research contexts)? {\bf Yes}\\
%Data and/or pretrained models are released under a specified license that is compatible with the conditions under which access to data was granted (in particular, derivatives of data accessed for research purposes should not be deployed in the real world as anything other than a research prototype, especially commercially)
%The paper specifies the efforts to limit the potential use to circumstances in which the data/models could be used safely (such as an accompanying data/model statement).
%The data is sufficiently anonymized to make identification of individuals impossible without significant effort. If this is not possible due to the research type, please state so explicitly and explain why.
%The paper discusses the harms that may ensue from the limitations of the data collection methodology, especially concerning marginalized/vulnerable populations, and specifies the scope within which the data can be used safely.
B4. Did you discuss the steps taken to check whether the data that was collected / used contains any information that names or uniquely identifies individual people or offensive content, and the steps taken to protect / anonymize it? {\bf NA.}\\
%There are some settings where the existence of offensive content is not necessarily bad (e.g., swear words occur naturally in text), or part of the research question (i.e., hate speech). This question is just to encourage discussion of potentially undesirable properties.
%Explain how you checked for offensive content and identifiers (e.g., with a script, manually on a sample, etc.).
%Explain how you anonymized the data, i.e., removed identifying information like names, phone and credit card numbers, addresses, user names, etc. Examples are monodirectional hashes, replacement, or removal of data points. If anonymization is not possible due to the nature of the research (e.g., author identification), explain why.
%List any further privacy protection measures you are using: separation of author metadata from text, licensing, etc.
%If any personal data is used: the paper specifies the standards applied for its storage and processing, and any anonymization efforts.
%If the individual speakers remain identifiable via search: the paper discusses possible harms from misuse of this data, and their mitigation.
B5. Did you provide documentation of the artifacts, e.g., coverage of domains, languages, and linguistic phenomena, demographic groups represented, etc.? {\bf NA}\\
%Be sure to report the language of any language data, even if it is commonly-used benchmarks.
%Describe basic information about the data that was used, such as the domain of the text, any information about the demographics of the authors, etc.
B6. Did you report relevant statistics like the number of examples, details of train / test / dev splits, etc. for the data that you used / created? {\bf Yes}\\
%Even for commonly-used benchmark datasets, include the number of examples in train / validation / test splits, as these provide necessary context for a reader to understand experimental results. For example, small differences in accuracy on large test sets may be significant, while on small test sets they may not be.\\
C. Did you run computational experiments? {\bf Yes}\\
C1. Did you report the number of parameters in the models used, the total computational budget (e.g., GPU hours), and computing infrastructure used? {\bf Yes}\\
%Even for commonly-used models like BERT, reporting the number of parameters is important because it provides context necessary for readers to understand experimental results. The size of a model has an impact on performance, and it shouldn’t be up to a reader to have to go look up the number of parameters in models to remind themselves of this information.
%The total computational budget can be presented however is most appropriate for the paper – if most experiments were run on GPUs, then important information would likely include the total number of GPU hours, the amount of parallelism across GPUs, the size of the GPUs, etc. to allow a reader to estimate the computational requirements to reproduce, use, or build upon the work.
%Note that this should include information about all experiments, not just the final runs that led to the results presented in the paper. If exact numbers are not available, an estimate is better than nothing.
C2. Did you discuss the experimental setup, including hyperparameter search and best-found hyperparameter values? {\bf Yes}\\
%The experimental setup should include information about exactly how experiments were set up, like how model selection was done (e.g., early stopping on validation data, the single model with the lowest loss, etc.), how data was preprocessed, etc.
%Many research projects involve manually tuning hyperparameters until some “good” values are found, and then running a final experiment which is reported in the paper. Other projects involve using random search or grid search to find hyperparameters. In all cases, report the results of such experiments, even if they were stopped early or didn’t lead to your best results, as it allows a reader to know the process necessary to get to the final result and to estimate which hyperparameters were important to tune.
%Be sure to include the best-found hyperparameter values (e.g., learning rate, regularization, etc.) as these are critically important for others to build on your work.
%The experimental setup should likely be described in the main body of the paper, as that is important for reviewers to understand the results, but large tables of hyperparameters or the results of hyperparameter searches could be presented in the main paper or appendix.
C3. Did you report descriptive statistics about your results (e.g., error bars around results, summary statistics from sets of experiments), and is it transparent whether you are reporting the max, mean, etc. or just a single run? {\bf Yes}\\
%Error bars can be computed by running experiments with different random seeds, Clopper–Pearson confidence intervals can be placed around the results (e.g., accuracy), or expected validation performance can be useful tools here.
%In all cases, when a result is reported, it should be clear if it is from a single run, the max across N random seeds, the average, etc.
%When reporting a result on a test set, be sure to report a result of the same model on the validation set (if available) so others reproducing your work don’t need to evaluate on the test set to confirm a reproduction.
C4. If you used existing packages (e.g., for preprocessing, for normalization, or for evaluation), did you report the implementation, model, and parameter settings used (e.g., NLTK, Spacy, ROUGE, etc.)? {\bf Yes}\\
%The version number or reference to specific implementation is important because different implementations of the same metric can lead to slightly different results (e.g., ROUGE).
%The paper cites the original work for the model or software package. If no paper exists, a URL to the website or repository is included.
%If you modified an existing library, explain what changes you made.
D. Did you use human annotators (e.g., crowdworkers) or research with human participants? {\bf No.}\\
%D1. Did you report the full text of instructions given to participants, including e.g., screenshots, disclaimers of any risks to participants or annotators, etc.?\\
%Examples of risks include a crowdsourcing experiment which might show offensive content or collect personal identifying information (PII). Ideally, the participants should be warned.
%Including this information in the supplemental material is fine, but if the main contribution of your paper involves human subjects, then we strongly encourage you to include as much detail as possible in the main paper.
%D2. Did you report information about how you recruited (e.g., crowdsourcing platform, students) and paid participants, and discuss if such payment is adequate given the participants’ demographic (e.g., country of residence)?\\
%Be explicit about how you recruited your participants. For instance, mention the specific crowdsourcing platform used. If participants are students, give information about the population (e.g., graduate/undergraduate, from a specific field), and how they were compensated (e.g., for course credit or through payment).
%In case of payment, provide the amount paid for each task (including any bonuses), and discuss how you determined the amount of time a task would take. Include discussion on how the wage was determined and how you determined that this was a fair wage.
%D3. Did you discuss whether and how consent was obtained from people whose data you’re using/curating? For example, if you collected data via crowdsourcing, did your instructions to crowdworkers explain how the data would be used?\\
%D4. Was the data collection protocol approved (or determined exempt) by an ethics review board?\\
%Depending on the country in which research is conducted, ethics review (e.g., from an IRB board in the US context) may be required for any human subjects research. If an ethics review board was involved, you should clearly state it in the paper. However, stating that you obtained approval from an ethics review board does not imply that the societal impact of the work does not need to be discussed.
%For initial submissions, do not include any information that would break anonymity, such as the institution conducting the review.
%D5. Did you report the basic demographic and geographic characteristics of the annotator population that is the source of the data?\\
%State if your data include any protected information (e.g., sexual orientation or political views under GDPR).
%The paper is accompanied by a data statement (see Bender and Friedman, 2018) describing the basic demographic and geographic characteristics of the author population that is the source of the data, and the population that it is intended to represent.
%If applicable: the paper describes whether any characteristics of the human subjects were self-reported (preferably) or inferred (in what way), justifying the methodology and choice of description categories.


==> disc.tex <==
\section{Discussion and Analysis}
\label{sec:discussion}



==> exp.0.tex <==
\section{Experimental Setup}
\label{sec:expt}

%\begin{comment}
\begin{table*}[ht]
\begin{center}
\small
%\resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{|c|l|ccc|ccc|ccc|}
%\toprule
%\textbf{Memory} & \textbf{Approach} & \multicolumn{5}{c}{\textbf{Datasets}} \\ 
\hline

  \multicolumn{1}{|c}{Train}&\multicolumn{1}{|c}{Model}&\multicolumn{3}{|c}{All}
  & \multicolumn{3}{|c}{Answerable}  & \multicolumn{3}{|c|}{Unanswerable}  \\
 
    
 & & F1(L) & F1(R) & EM & F1(L) & F1(R) & EM & F1(L) & F1(R) & EM \\ \hline
  \multirow{4}{*}{A}&RnG-KBQA & 67.8 &65.6  &51.5  & {\bf 78.1}  & {\bf 78.1}  & {\bf 74.2}  &46.9  &40.3  & 5.7 \\ 
 &RnG-KBQA+T & 67.6 &65.8  &56.9  & 71.4 &  71.3& 68.5 & 59.9 &54.5  &33.5  \\ 
  &ReTraCk &69.3 &67.1 &50.7  &67.0  &66.9  &62.4  &73.9  &67.3  &27.2  \\

   &ReTraCk+T &69.9  &67.9  &52.0  &65.3  &65.3  &61.2 &79.3  &73.2  &33.5  \\
  \hline 
  \multirow{4}{*}{A+U}&RnG-KBQA & {\bf 80.5} & {\bf 79.4} & {\bf 68.2}  &75.9  &75.9  &72.6  &89.7  &86.4  &59.4  \\ 
 &RnG-KBQA+T & 77.8 &77.1  &67.8  &70.9  &70.8  & 68.1 & {\bf 92.0}  & {\bf 89.8}  & {\bf 67.1}  \\ 
  &ReTraCk &69.7  &68.4  &56.5  &61.4  &61.3  &57.3  &86.4  &82.8  &54.8  \\
  &ReTraCk+T &70.3  &69.1 &56.6  &61.2  &61.1  &57.1  &88.7  &85.1  &55.5  \\
  \hline 
\end{tabular}
%}
\end{center}
\caption{Performance of different models on GrailQAbility over all, answerable and unanswerable questions. EM is exact match on logical forms and F1(L) and F1(R) are lenient and regular evaluations of answers. A and A+U indicate training with only answerable questions and with both answerable and unanswerable questions. Models with suffix +T have additional thresholds for entity linking and LF generation fine-tuned on GrailQAbility dev set.}
\label{tab:mainresult}
%\vspace{-0.5cm}
\end{table*}


\begin{table*}[ht]
        \begin{center}
            \small
            % \scriptsize
            %\resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{|c|l|cccccc|cccc|}
%\toprule
%\textbf{Memory} & \textbf{Approach} & \multicolumn{5}{c}{\textbf{Datasets}} \\ 
\hline
  \multicolumn{1}{|c}{Train}&\multicolumn{1}{|c}{Model}&\multicolumn{6}{|c}{Schema Element Missing}  
  & \multicolumn{4}{|c|}{Data Element Missing}  \\     
  & &\multicolumn{2}{c}{Type}  
  & \multicolumn{2}{c}{Relation}  & \multicolumn{2}{c|}{Mention Entity} &
  \multicolumn{2}{c}{Other Entity} &
  \multicolumn{2}{c|}{Fact}  \\     
  & & F1(R) & EM &  F1(R) & EM  & F1(R) & EM &F1(R) & EM & F1(R) & EM  \\ \hline
  \multirow{3}{*}{A}&{\small RnG-KBQA} & 40.1  &0.0    &44.2  & 0.0   &27.2  &0.0 &45.1  & 13.5   &46.2  &16.9 \\ 
 &{\small RnG-KBQA+T}  &55.5  &49.5    &57.1  &46.6    &44.4  & 40.1  &56.0  & 11.5& 58.7  &14.1 \\ 
  &{\small ReTraCk}   &71.1  &34.8    &59.3  &18.9    &80.8  &63.9 &72.6  &11.2   &64.5  &12.2 \\

   &{\small ReTraCk+T}   &75.7  &47.9 &64.9  &28.8    &83.6  &70.4 &81.0  &10.9   &72.4  &12.3 \\
  \hline 
  \multirow{3}{*}{A+U}&{\small RnG-KBQA}  &91.6  &75.8& 86.4 & 66.6   &87.5  &72.0&84.0  & {\bf 37.5}   &82.5  & {\bf 39.3}  \\ 
 &{\small RnG-KBQA+T}   & {\bf 93.4}  & {\bf 86.8}    & {\bf 89.7}  & {\bf 85.5}    & {\bf 92.0}  & { \bf 89.5} & {\bf 87.1}  &30.8  & {\bf 86.0}  &32.7 \\ 
  &{\small ReTraCk}   &89.6  &82.2    &86.4  &74.4    &90.3  &85.9   &79.0  &9.8    &71.7  &11.0 \\
  &{\small ReTraCk+T}   &90.6  &83.1    &87.8  &76.0    &91.2 &86.9 &83.2  &9.8 &76.3  &11.0 \\
  \hline 
\end{tabular}
%}
\end{center}
\caption{Performance for different KBQA models for subsets of questions affected by different types of KB incompleteness. 
Note that missing mention entities result in invalid logical form and other missing entities lead to valid logical form with no answer. 
Names have the same meanings as in Tab.~\ref{tab:mainresult}.}
\label{tab:drop_type}
%\vspace{-0.5cm}
\end{table*}


\begin{table}[ht]
\begin{center}
\small            %\resizebox{1\linewidth}{!}{
\begin{tabular}[b]{|c|l|cc|cc|}
%\toprule
%\textbf{Memory} & \textbf{Approach} & \multicolumn{5}{c}{\textbf{Datasets}} \\ 
\hline
  \multicolumn{1}{|c}{Train}&\multicolumn{1}{|c}{Model}
  
  & \multicolumn{2}{|c}{Full Z-Shot }  & \multicolumn{2}{|c|}{Partial Z-Shot}  \\ 
 
    
 &  & F1(R) & EM & F1(R) & EM \\ \hline
  \multirow{3}{*}{A+U}&RnG-KBQA     &87.5  &75.4 &79.1  &44.5 \\ 
 &RnG-KBQA+T    & {\bf 89.5}  & {\bf 85.1} & {\bf 83.6}  & {\bf 68.2}   \\ 
  &ReTraCk     &84.3  &62.1 &74.8  &53.5  \\
  &ReTraCk+T      &87.9  &63.7  &76.7  &55.4 \\
  \hline 
\end{tabular}
%}
\end{center}
\caption{Performance of different models for partial zero-shot and full-zero test scenarios in GrailQAbility. Names have the same meanings as in Tab.~\ref{tab:mainresult}.}
\label{tab:zeroshot_drilldown}
%\vspace{-0.5cm}
\end{table}




\begin{comment}
    

\begin{table*}[ht]
        \begin{center}
            \small
            % \scriptsize
            %\resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{|c|l|ccc|ccc|ccc|ccc|}
%\toprule
%\textbf{Memory} & \textbf{Approach} & \multicolumn{5}{c}{\textbf{Datasets}} \\ 
\hline
  \multicolumn{1}{|c}{Train}&\multicolumn{1}{|c}{Model}&\multicolumn{3}{|c}{Type Drop}  
  & \multicolumn{3}{|c}{Relation Drop}  & \multicolumn{3}{|c}{Entity Drop} & \multicolumn{3}{|c|}{Fact Drop}  \\     
 & & F1(L) & F1(R) & EM & F1(L) & F1(R) & EM & F1(L) & F1(R) & EM& F1(L) & F1(R) & EM  \\ \hline
  \multirow{3}{*}{A}&{\scriptsize RnG-KBQA} & 47.7 &42.6  &0.0  &60.0  &51.0  & 0.0 &36.5  &31.9  &6.6 &53.6  &42.1  &13.9 \\ 
 &{\scriptsize RnG-KBQA+T} &65.3 &61.3  &47.9  &70.5  &62.3  &39.7  &52.0  &48.8  & 27.0& 65.3 &56.2  &11.3 \\ 
  &{\scriptsize ReTraCk} &78.8  &74.9  &33.6  &73.9  &63.7  &15.1  &82.7  &80.1  &43.5 &76.7  &69.7  &9.5 \\

   &{\scriptsize ReTraCk+T} &84.5  &81.2  &42.3  &79.9  &69.9  &22.9  &84.6  &82.0  &46.3 &76.7  &69.6  &9.5 \\
  \hline 
  \multirow{3}{*}{A+U}&{\scriptsize RnG-KBQA} & 92.5 &89.8  & 76.0 &88.5  &82.8  &64.4  & 84.0 &81.5  &50.1 &83.3  &76.5  &{\bf 35.0}  \\ 
 &{\scriptsize RnG-KBQA+T} &95.1  &92.7  &89.0  &90.6  &85.4  &{\bf 80.1}  &88.7  &87.2  &61.0 &{\bf 85.8}  &{\bf 80.4}  &27.9 \\ 
  &{\scriptsize ReTraCk} &{\bf 98.6}  &{\bf 97.8}  &{\bf 94.9}  &{\bf 92.8}  &{\bf 88.1}  &75.8  &{\bf 90.9}  &{\bf 89.2}  &53.4  &85.7  &79.6  &9.5 \\
  &{\scriptsize ReTraCk+T} &{\bf 98.6}  &{\bf 97.8}  &{\bf 94.9}  &{\bf 92.8}  &{\bf 88.1}  &75.8  &{\bf 90.9}  &{\bf 89.2}  &53.4  &85.7  &79.6  &9.5 \\
  \hline 
\end{tabular}
%}
\end{center}
\caption{Performance for different KBQA models for subsets of questions affected by different types of KB incompleteness. Names have the same meanings as in Tab.~\ref{tab:mainresult}.}
\label{tab:drop_type}
%\vspace{-0.5cm}
\end{table*}
\end{comment}
%We now discuss the KBQA models that we choose for experimentation and how we adapt these for detecting answerability.

%Our dataset GrailQAbility is the first KBQA benchmark with unanswerable questions.
%Since there are no KBQA models that address unanswerability, we experiment with state-of-the-art models and investigate their ability to address the task of KBQA with answerability detection with appropriate retraining.
%Since these models assume answerability of questions, their design is not expected to be naturally robust against unanswerability. 
%Nevertheless, the study of different existing KBQA architectures on GrailQAbility is a natural first step towards the design of better models for unaswerability detection.

%\subsection{KBQA Models and Training}
\paragraph{KBQA Models:}
Among state-of-the-art KBQA models, we pick RnG-KBQA~\cite{ye:acl2022rngkbqa} and ReTraCk~\cite{chen:acl2021retrack}.
These report state-of-the-art results on GrailQA as well as on WebQSP~\cite{berant-etal-2013-semantic,yih:acl2016webqsp,talmor:acl2018complexwebqsp} - the two main benchmarks.
On the GrailQA leader board,\footnote{\url{https://dki-lab.github.io/GrailQA/}} these are among the top three published models  with available code.
Since these generate logical forms, we expect these to be more robust to data level incompleteness than purely retrieval-based approaches~\cite{saxena:acl2020kgqaembed,das:emnlp2021cbr,zhang:acl2022subgraph,mitra:naacl2022cmhopkgqa,wang:naacl2022mhopkgqa}. 
%Also, importantly, these have important differences in their architecture, relevant for answerability.
%We expect the sketch generation based approach~\cite{cao:acl2022progxfer} also to have some ability to detect answerability but unfortunately this does not have working code available yet~\footnote{\url{https://github.com/THU-KEG/ProgramTransfer}}.

%\paragraph{RnG-KBQA~\cite{ye:acl2022rngkbqa}} 
{\bf RnG-KBQA~\cite{ye:acl2022rngkbqa}} 
%It's generation augmented iterative ranking-based approach where given each mentioned entity in the question they enumerate all data level paths up to 2-hops and convert them into s-expressions (candidate logical forms). These candidate logical forms are ranked by the ranker and then top-k candidate logical forms along with the question are used to generate the target logical form. 
follows a rank and generate approach, where a BERT-based ~\cite{Devlin2019BERTPO} ranker selects a set of candidate logical forms for a question by searching the KB, and then a T5-based ~\cite{2020t5} model generates the logical form using the question and candidates.  
%It also uses the same ranking approach to perform entity linking.
%We use existing code from github \footnote{\tiny{\url{https://github.com/salesforce/rng-kbqa}}} and augment the entity disambiguation and generator module with thresholding.
%with a function which can now return respective outputs along with the score. Due to presence of NA questions, instead of execution-guidance we select logical form based on the perplexity score.
%What changes do we make? 
%Threshold?
%\paragraph{ReTraCk~\cite{chen:acl2021retrack}}
{\bf ReTraCk~\cite{chen:acl2021retrack}} also uses a rank and generate approach, but uses a dense retriever to retrieve schema elements for a question, and grammar-guided decoding using an LSTM ~\cite{lstm} to generate the logical form using the question and retrieved schema items.
%We use the pre-trained entity linker as used in the original paper.
%We use existing code from github \footnote{\tiny{\url{https://github.com/microsoft/KC/tree/main/papers/ReTraCk}}}.
%We augment the grammar to enable the generation of NK.
%Each logical form is associated with a score, we use it to decide a threshold and convert below threshold logical forms to NK.
Both models check execution for generated logical forms.
%Since the generator does not ensure validity of the logical form, it uses execution-guidance to select the top valid logical form.
%It additionally uses instance and ontology-level checking and real and virtual execution to improve decoder performance.


\paragraph{Adapting for Answerability:} 
We use existing codebases\footnote{\url{https://github.com/salesforce/rng-kbqa}}\footnote{\url{https://github.com/microsoft/KC/tree/main/papers/ReTraCk}} %and augment with thresholding for entity disambiguation and logical form generation.
of both models, which we adapt for our task in two different ways.
ReTraCk returns empty logical form when execution fails, which we interpret as $l=\mbox{NK}$ prediction.
Additionally, %we use thresholding on output probability for both models to generate $\mbox{NK}$ predictions.
%Specifically, 
we introduce two different thresholds for entity disambiguation and logical form, and take the prediction to be $\mbox{NK}$ when MAP probabilities for entity disambiguation and logical form are less than their corresponding thresholds. 
These thresholds are tuned using the validation set.
%\paragraph{Training with Unanswerability: }
%{\bf Training with Unanswerability: }
%While the test set contains both answerable and unanswerable questions, we train the chosen KG-QA model under two different settings.
For training, in the simplest setting ({\bf A training}), we train the models as in their original setting with only the answerable subset of training questions, leaving out the unanswerable questions.
%In this setting, RnG does not predict \textsc{NK} for the logical form, but we interpret ReTraCk's empty string prediction as \textsc{NK}. 
%ReTrack on the other hand would predict NK when the confidence is low.
%In the {\bf A} setting, the unanswerable questions are removed from the training set, and the model is trained only with answerable questions.
We also train by using both the answerable and unanswerable questions in  the training data ({\bf A+U training}).
%In the {\bf A+U} setting, the model is provided with both answerable and unanswerable questions in the training set.
%This enables both models to predict NK for the logical form.
%\paragraph{Thresholding: }
%{\bf Thresholding: }
%A possible indication of a question being unanswerable is that the model is uncertain about its predicted answer, or in other words the most likely answer has low probability.
%Such selective answering has been explored for QA in the context of answer classification~\cite{kamath:acl2020-selective}.
%However, thresholding on probabilities does not work for KG-QA models that output variable-length programs, instead of answers.
%For such models, we compute a threshold on perplexity instead of probability by tuning on the validation set.
%Both models follow a pipeline approach that first performs entity linking and later logical form generation.
%Low confidence in both steps is an indication of the question being unanswerable.
%We add thresholds to these decisions - $\tau_e$ for entity linking and $\tau_l$ for logical form - and fine-tune these thresholds on the validation set (with or without training with unanswerability). 
%We now take the models prediction to be NK for the logical form when (a) the actual prediction is NK, (b) the entity linking confidence is less than $\tau_e$, OR (c) the logical form confidence is less than $\tau_l$.  
More details on their adaptation are in appendix (\ref{sec:traindetails}).


%\subsection{Evaluation Measures}
%\paragraph{Evaluation Measures}
%Some of the models directly generate the answer, while others generate the logical form, and the answer is obtained by executing the logical form.
%The datasets have gold labels for both the logical form and the answer. 
%So we evaluate the models for the answer and for the logical form, where applicable.
%While predicting answers is the end goal in KBQA, both models under consideration are directly responsible only for generating the logical form, which is executed by a query engine to produce answers.
%Further, the logical form provides the explanation behind the answer (or no-answer).
%In the context of answerability, it is important to distinguish, for example,  between NK or a valid logical form accompanying NA as the answer.
%So 
%We evaluate both the answers and the logical form.
%\paragraph{Answer Evaluation:} 
%{\bf Answer Evaluation:} 
%Since a question may have multiple answers, we evaluate predicted answers using precision, recall and F1 ~\cite{ye:acl2022rngkbqa}.
%In regular answer evaluation (R), we compare the predicted answer for a question $q$ only with its possibly modified gold answer $a_{au}$ in the unaswerability dataset $Q_{au}$. %with unanswerable questions $D_u$.
%However, some model may still be able to predict the `ideal' answer $a$ for $q$ in the original dataset $Q$, perhaps by inferring missing facts.
%To give credit to such models, we propose a lenient answer evaluation (L), where we compare the predicted answer against both $a_{au}$ and $a$.
%Details of lenient evaluation measure are in the appendix \ref{sec:lenientevaluation}.
%However, we do evaluations at different levels of strictness.
%For very strict evaluation (VS), in addition to checking the predicted answer with the gold answer, we also check if the logical form is correct.
%In other words, the answer as well as the explanation matches the gold standard.
%For strict evaluation (S), we only compare the predicted answer with the gold standard answer.
%However, here the predicted answer is penalized for an unanswerable question even when it matches the answer for the original answerable question.
%We account for this in the lenient (or not strict) evaluation (NS) by rewarding the answers that match the gold-standard answer OR the original answer if different from the gold-standard.
%\paragraph{Logical Form Evaluation:}
%{\bf Logical Form Evaluation:}
%For models that generate the logical form, 
%For evaluating logical forms, as usual, we compare the predicted logical form with the gold-standard one in $Q_{au}$ using exact match (EM)~\cite{ye:acl2022rngkbqa}.

\paragraph{Evaluation Measures: }
To evaluate a model's performance for detecting unanswerability, we primarily focus on the correctness of the logical form. 
We compare the predicted logical form with the gold-standard one using exact match (EM)~\cite{ye:acl2022rngkbqa}.
%For questions having valid logical forms but no answer, it is also important to evaluate the answer.
As it is ultimately a QA task (and other systems may produce answers without generating logical forms), we also define metrics for direct answer evaluation.
Since in general a question may have multiple answers, we evaluate predicted answers using precision, recall and F1 ~\cite{ye:acl2022rngkbqa}.
In regular answer evaluation (R), we compare the predicted answer only with the gold answer in the modified KB, as usual.
We also consider a lenient answer evaluation (L) for our setting, where we account for the gold answer in the original (ideal) KB as well, and also give credit to models which are able to recover the old answer, perhaps via inference.
As an example, for the second test question in Fig.~\ref{fig:example}(C), R-evaluation would only reward $\mbox{NA}$ as answer, whereas L-evaluation would reward both $\mbox{NA}$ and {\em USA} as perfect answers.
Details of evaluation measures are in appendix (\ref{sec:lenientevaluation}).

%\subsection{Results}

